2PPS -- Publish/Subscribe with Provable Privacy

Publish/Subscribe systems like Twitter and Reddit let users communicate with many recipients without requiring prior personal connections. The content that participants of these systems publish and subscribe to is typically public, but they may nevertheless wish to remain anonymous. While many existing systems allow users to omit explicit identifiers, they do not address the obvious privacy risks of being associated with content that may contain a wide range of sensitive information. We present 2PPS (Twice-Private Publish-Subscribe), the first pub/sub protocol to deliver strong provable privacy protection for both publishers and subscribers, leveraging Distributed Point Function-based secret sharing for publishing and Private Information Retrieval for subscribing. 2PPS does not require trust in other clients and its privacy guarantees hold as long as even a single honest server participant remains. Furthermore, it is scalable and delivers latency suitable for microblogging applications. A prototype implementation of 2PPS can handle 100,000 concurrent active clients with 5 seconds end-to-end latency and significantly lower bandwidth requirements than comparable systems.

==> sections/Multiple_Blocks_Retrieval.tex <==
% Multiple Blocks Retrieval

\textbf{\textit{Problem definition:}}
In the traditional PIR method, the client can retrieve $M$ blocks from $S$ servers by sending  $M*S$ PIR queries. That induces communication overhead. Additionally, it allows the adversary to learn the exact number of blocks that the client is interested in.
 
The goal is to allow the client to retrieve many blocks using only $S$ PIR queries. 

\textbf{\textit{Assumptions:}}
\begin{itemize}
\item There are $S$ servers where each one of them stores the same copy of the database.
\item The database consists of $n$ equal-sized blocks. 
\item The size of the block is $b$ bits.
\item Blocks will be grouped into $h$ buckets. 
\item The number of blocks per bucket is $z$, where $n/z$ must be an integer. 
\item In the traditional case, the bucket size equals one that means there is only one block per bucket. 
\end{itemize}

\textbf{\textit{Solution:}}
Client-side:
\begin{itemize}
\item Choose the value of $z$. 
\item Create a binary vector $q$ of size $n$, and put 1 in the index of each block that she wants to retrieve. She should know that she can’t retrieve the $i$th block (e.g., the first block) in both bucket $A$ and bucket $B$. In other words, she can only retrieve blocks in different positions in the buckets.   
\item Create $S-1$ random vectors of size $n$.  
\item XOR the random vectors from step 3 with $q$.
\item Send $S-1$ vectors from step 3 and the result of step 4 to servers where each server gets only one vector.
\item After the client receives the responses from the servers, she XORs all of them to get the final reply. 
 \end{itemize}
 
Server-side:
\begin{itemize}
\item Compute the PIR response by XORing all the buckets that have blocks with 1 in their positions in the received vector. 
\item The server sends a reply of size $z*b$ bit to the clients.
\end{itemize}

To minimize the padding and to have variable block-size, blocks in the bucket can have different sizes. However, the size of block $i$ in every bucket should be the same. 


==> sections/attacks.tex <==
\section{Attacks}
% This draft gives info about possible attacks in our system. This could be a separate section or subsection in another section.

\subsection{Traffic Analysis Attacks}
In 2PPS, we aim to prevent traffic analysis attacks. To achieve this, communication is carried out in rounds, similar to previous designs with traffic analysis resistance [RefRiffle, RefRiposte, and RefDissent]. In each round, every online client sends and receives a message, even if he or she does not wish to communicate that round. The difference between our system and other traffic analysis resistance systems is that we don’t force clients to be online all the time. We increase the anonymity set of publishers by making subscribers participating in writing rounds.  That leads to having a big anonymity set since the number of subscribers in 2PPS is much larger than the number of publishers.
%mention dummy subscriptions

\subsection{Attacks against the availability}
%mention auditing to defend against DoS by clients
%drop shares by malicious servers
% wrong PIR replies by malicious servers 
% Corrupt reply by server P

\subsection{Active Attacks}
The basic 2PPS has a weakness against active attacks that try to link senders to their messages, which is inherent from the public nature of all messages.
The adversary can interfere with the messages of the target client and observe the consequences of his actions after publishing.
\paragraph*{Replay}
An intuitive example for these attacks is based on replaying:
$\mathcal{A}$ saves all DPF-shares Alice sends in a given round and all message that are revealed in the same round.
In the next round, $\mathcal{A}$ inserts the saved shares into the traffic.
the servers will add them to their $db_w$ state.
$\mathcal{A}$ can identify which messages Alice has sent by observing which identical message was revealed in both rounds.
To detect replayed messages, Alice includes the current round number with every DPF-share.
A honest servers can check the include round number for currentness and refuse further participation if this check fails.
DPF-shares and round number are encrypted with the public key of the receiving server to prevent $\mathcal{A}$ from modifying the round number of the replayed messages.
$\mathcal{A}$ could also replay the shares in the same round as the original shares, which would corrupt Alice's message.
However, this attack is easily detectable by the honest server, since it has access to all shares of the current round at once and can check for duplicates.


% Intersection attacks typically become more difficult to mount as the size of the anonymity set increases, so 2PPS's support for very large anonymity sets makes it less vulnerable to these attacks than are many other systems.

\subsection{Intersection Attacks}
Intersection attacks allow a global adversary or an adversary who controls one of 2PPS severs to link a targeted client to her topic or even published message. To perform such an attack, when a client sends a message, the adversary records the topics of messages in this round.  One of these topics could potentially have been the topic of the client’s message. This is done repeatedly until the intersection of all the potential topics reveals a single topic or a small set of topics that with high probability includes the client’s interest(s)/topic(s).

This attack represents a serious issue especially in systems like 2PPS where messages could be public (like in microblogging application scenario), and when we have a high churn rate in the user base of an ACS. Churn is something natural in communication systems where over time new clients may join the system whereas other clients may stop using the service altogether. Also, clients may start to post at different times which make messages linkable via statistical disclosure and intersection attacks eventually. 

The aim of any anonymous communication system that resists intersection attacks is to delay this anonymity degradation process. We believe that security based on the assumption of constant client participation (like in Express, Riffle, Vuvuzela, Riposte) is impractical and makes the anonymity system less usable. Also, the constant client participation might not prevent the adversary from differentiating between the behavior of old clients and new clients.

To mitigate the intersection attacks in 2PPS and provide a practical solution at the same time, we use:
\begin{enumerate}
\item Cover traffic \& big anonymity set: When the client is online, she will participate in all rounds by either sending a real or cover message. Even if the client is just a subscriber and not a publisher, she still must participate in writing rounds as long as she is online. That leads to a very big anonymity set of publishers because the number of subscribers is usually much larger than the number of publishers.
\item Delay: If the client can tolerate latency, she will include a delay with her private write request.  This will be done as follows:
\begin{itemize}
\item Before passing m to Gen function, the client adds delay value $d$ to $tm|m$, and encrypts the result using the public key of one of the servers (randomly chosen).
\item After servers combine their databases, each server will try to find all messages that are encrypted using its public key to decrypt them and move them to its copy of $db_r$.
\item Servers will share their copy of $db_r$ state and combine them to produce the final copy of $db_r$.
\end{itemize}
\end{enumerate}

Clients don't need to include delays in their messages every round. Also, not all of them need to do that together.  If just part of clients added delay to their messages, that would make the intersection attack harder since the adversary could not tell who exactly included delay and who didn't in round r. 
Using this method,  each server will know the topics of some of the submitted messages. If the malicious servers collude, this will reveal the topics of more messages. However, the topics of some messages will be secret because one of the servers is honest. 

By relying on DPF to break the link between the client and her message, and the delay to break the link between the submitting time and the publishing time,  it will not be easy to know when the client’s message will appear. Therefore, the adversary will not be able to learn the list of the active topics when the client's message will be published.








==> sections/background.tex <==
\section{Background}
%\subsection{Pub/Sub}
%Our system aims to provide open group communication between several untrusted users. The topic-based pub/sub messaging model fits this setting. It supports a loose coupling between publishers (message writers) and subscribers (message readers) of a topic. Publishers write messages to a topic which acts like a channel. The subscribers of this topic are listening to the channel and are notified of new messages.
%To decouple the publishers and subscribers, third party servers are commonly used. They handle read/write requests from the clients and manage the topics \cite{Refpubsub}. Therefore, intermediate servers have knowledge of the communication and can gather important information about the publishers and subscribers.
%\cc{I don't think we need a pub/sub section when we already explain the basics in the introduction}
We provide some background on the building blocks of 2PPS:
Distributed point function-based secret sharing for anonymous publishing of messages and information-theoretic private information retrieval for anonymous subscription.
\subsection{Secret Sharing \& DPF}
We present some background on secret sharing and distributed point functions based on Express~\cite{RefExpress}.
Assume that client $u$ wants to write message $m$ at index $i^\ast$ to a database of $\ell$ elements that is distributed among two servers.
The client wants to do so without revealing to the servers which index he has written his message to.
Consider the following na\"ive approach:
\begin{enumerate}
    \item $u$ creates a vector $m \cdot \mathbf{e}_{i^\ast} \in \mathbb{F}^\ell$, where $\mathbf{e}_{i^\ast}$ is a vector that has zeros in all positions in $\mathbb{F}^\ell$ except in the position $i^\ast$ where it is equal to $1$. 
    \item $u$ chooses a random $w_1\in \mathbb{F}^\ell$ and computes $w_2\in\mathbb{F}^\ell$ such that $w_1+w_2=m \cdot \mathbf{e}_{i^\ast}$
    \item $u$ sends $w_j$ for $j\in\{1,2\}$ to server $S_j$, which adds it to its database state $D_j$:
\end{enumerate}
\begin{align*}
    D_j \gets D_j + w_j
\end{align*}

After processing requests from multiple clients, the servers can collaborate to compute a combined database $D = \sum_{j} D_j$.
As long as every client chose a unique index for her messages, $D$ contains all original messages.
Since individual shares appear random and messages are revealed all at once, an adversary is not able to link any message to its original sender.

While this na\"ive solution ensures client privacy, it is very inefficient:
For every write request, a vector with the same size as the database has to be sent.
To address this issue,  Riposte~\cite{RefRiposte} suggested the use of distributed point functions (DPF).
\begin{definition}[DPF]
    Let $f_{i^\ast,m} : \{0,\dots,\ell\} \mapsto \mathbb{F}$ be a point function with
    \begin{align*}
        f_{i^\ast,m}(i) &= \begin{cases}
            m &\text{for } i = i^\ast\\
            0 &\text{for } i\in\{0,\dots,\ell\}\setminus i^\ast
        \end{cases}
    \end{align*}
    $f_A, f_B : \{0,\dots,\ell\} \mapsto \mathbb{F}$ are distributed point functions of $f_{i^\ast,m}$, iff
    \begin{enumerate}
        \item Neither $f_A$ nor $f_B$ by themselves reveal anything about $m$ or $i^\ast$
        \item $\forall\: i\in \{0,\dots,\ell\} : f_A(i) + f_B(i) = f_{i^\ast,m}(i)$
    \end{enumerate}
\end{definition}

DPFs can be used to \emph{compress} the shares sent to the servers from the na\"ive approach:
To send message $m$, the client chooses a random index $i^\ast$ and computes the DPFs $f_A,f_B$ corresponding to $f_{i^\ast,m}$ as defined above.
$f_A$ is sent to the first server and $f_B$ is send to the second server.
Each server can evaluate its share at every point $i\in\{0,\dots,\ell\}$ to recreate $w_i$.
Current research states that sending a DPF share instead of $w_i$ directly reduces the communication cost to $O(\lambda\cdot\log \ell + \log |\mathbb{F}|)$ bits where $\lambda$ is the security parameter~\cite{RefFSS}.

\subsection{IT-PIR}
Information-theoretic private information retrieval (IT-PIR) \cite{RefITPIR1, RefITPIR2, RefITPIR3} allows a client to read from a remote database at a chosen index without revealing to the owner of the database which index she is interested in.
In most IT-PIR schemes, trust is distributed among several servers which each maintain a copy of the whole database.
As long as at least one server is honest and does not collude with the other servers, the user's privacy is protected.

To illustrate the concept of IT-PIR, let us consider a client $u$ who wants to read from a database $D$ consisting of $\ell$ elements at index $i^\ast\in\{0,\dots,\ell\}$.
We assume $n$ servers $S_1,\dots,S_n$, each maintaining a copy of the database $D$.
The client then takes the following steps:
\begin{enumerate}
\item $u$ generates an interest vector $q = (q_0,q_1,\dots,q_\ell)$, which is equal to $0$ in all components but the $i^\ast$th one
\item $u$ generates $n-1$ random vectors $p_1, p_2, p_3,\dots, p_{n-1}$
\item $u$ sends request $p_j$ to server $S_j$
\item $u$ sends request $p_n = p_1 \oplus p_2 \oplus p_3 \oplus \cdots\oplus p_{n-1} \oplus q$ to server $S_n$
\item Each server $S_j$ computes a response $r_j$, which is the XOR of all rows of $D$ that correspond to an 1-component of $v_j$.
    $r_j$ is then sent back to the client.
\item $u$ computes $m=r_1 \oplus r_2 \oplus \cdots \oplus r_n$
\end{enumerate}



==> sections/extensions.tex <==
\section{Protecting against Stronger Adversaries}

The basic 2PPS has a weakness against active attacks that try to link senders to their messages, which is inherent from the public nature of all messages.
The adversary can interfere with the messages of the target client and observe the consequences of his actions after publishing.
\paragraph*{Replay}
An intuitive example for these attacks is based on replaying:
$\mathcal{A}$ saves all DPF-shares Alice sends in a given round and all message that are revealed in the same round.
In the next round, $\mathcal{A}$ inserts the saved shares into the traffic.
the servers will add them to their $D_w$ state.
$\mathcal{A}$ can identify which messages Alice has sent by observing which identical message was revealed in both rounds.
To detect replayed messages, Alice includes a current timestamp with every DPF-share.
A honest servers can check the time stamp for currentness and refuse further participation if this check fails.
DPF-shares and round number are encrypted with the public key of the receiving server to prevent $\mathcal{A}$ from modifying the timestamp of the replayed messages.
$\mathcal{A}$ could also replay the shares in the same round as the original shares, which would corrupt Alice's message.
However, this attack is easily detectable by the honest server, since it has access to all shares of the current round at once and can check for duplicates.
\paragraph*{Modification}
Our proposed protection against replay attacks also enables honest servers to detect if a received request was modified by $\mathcal{A}$.
We assume that encryption used to protect the share and the timestamp provides \emph{diffusion}, i.e., ensures that any change of a ciphertexts leads to widespread and unforseable changes of the plaintext.
Thus, any modification of a request leads to a significant change of the included timestamp with overwhelming probability.
The honest server detects this invalid timestamp and refuse further participation in the current round.
\paragraph*{Drop \& Delay.}
Attacks based on dropping and delaying messages are both very common and hard to avoid in anonymous communication \cite{RefVuvuzela}.
If a powerful adversary is able to drop the requests of all but one client, then he can unambiguously link this client to her messages once the shares are combined.
A less powerful adversary might have insider knowledge of a message that will be sent in a given round.
For example, the leader of a group of political activists might plan to announce the start of a new protest against the regime.
The regime suspects that Alice is the leader and drops her message.
If the expected announcement does not happen, the regime's suspicion is confirmed and Alice may face prosecution.

Detecting malicious drops is not possible without making further assumptions, since user churn and drops due to technical problems prohibit honest servers from knowing the number of messages that are supposed to arrive in a given round.
Related literature commonly assumes that protocol participation is static, i.e., that clients are always online \cite{RefVuvuzela}.
This is a very strong and arguably not very realistic assumption, especially if clients rely on mobile devices.
We introduce an additional mechanism that enable us to make weaker assumptions regarding client participation:

The \emph{verifiable participation commitment} requires every client who joins the network to send a message to each server with which the client commits herself to participating in the next $k$ rounds.
The parameter $k$ can be chosen by the client to fit his routine.
A client could for example join when arriving at his office in the morning and commit to participate until his usual end of the work day.
Clients can also commit to shorter periods and renew their commitment periodically.
With that, the honest server knows from which clients to expect requests in any given round.
If less requests that expected arrive, the server assumes that a malicious drop must have occurred and refuses further participation to protect the senders privacy.
The adversary also needs to be prevented from replacing dropped requests with self-generated ones to circumvent the protection.
This can be done by requiring the clients to include a \emph{digital signature} with every request.
That way, each request can be linked to the client who sent it and the server can \emph{verify} that all committed clients have indeed participated.

%\section{Resisting Disruptions}
\paragraph*{Disruption by Clients.}
DPF-based secret sharing is not only vulnerable to disruption by servers but also by clients.
If a malicious client submits a malformed write request which contains non-zero values in more than one slot, this request is likely to cause collisions in the write database which make other messages unrecoverable.
To mitigate this issue, Riposte~\cite{RefRiposte} introduced an \emph{auditing} system which allows servers to confirm than an incoming share is not malformed (which was later improved upon by Express~\cite{RefExpress}).
The auditing protocol fulfills three requirements:
\begin{itemize}
    \item \textbf{Completeness}:
        If all participants are honest, the audit always accepts.
    \item \textbf{Soundness against malicious clients}:
        If a request is not valid and all servers are honest, the audit rejects with overwhelming probability.
    \item \textbf{Zero knowledge against malicious server}:
        A single malicious servers learns nothing about the request of an honest client by participating in the auditing protocolexcept the fact that the request is valid.
\end{itemize}
Express' variant of the auditing protocol uses secret-shared non-interactive proofs (SNIPs)~\cite{RefSNIP1,RefSNIP2} between the client sending the request and the servers.
Further details can be found in the Express paper~\cite{RefExpress}.

\begin{comment}  
\section{Extending Functionality}
\cc{
    I don't think that this fits well into the story.
    Also, we should be fine content-wise, so maybe we can just leave these extensions out..
}
\subsection{Closed Groups}
While 2PPS is primarily intended to provide communication through open groups, users might also want to have the possibility to exchange more sensitive information.
Without major changes to the protocol design, adversaries cannot be prevented to join groups (private topics may not be advertised, but joining by guessing subscription vectors is inevitable).
Message confidentiality can however be achieved trivially:
Assume that all group members trust each other and have agreed upon a shared secret key $k$.
This key can then be used to add an additional layer of encryption to messages of the confidential topic.
Note that only the message content, not the topic identifier may be encrypted.
Otherwise the servers would not be able to distinguish the confidential message from cover and discard it.
Subscribers to the confidential topic can use $k$ to reveal the content.

\subsection{Archive Retrieval}
TBD.
\end{comment}  


